Enhanced Detection of Transdermal Alcohol Levels Using Hyperdimensional Computing on Embedded Devices

Alcohol consumption has a significant impact on individuals' health, with even more pronounced consequences when consumption becomes excessive. One approach to promoting healthier drinking habits is implementing just-in-time interventions, where timely notifications indicating intoxication are sent during heavy drinking episodes. However, the complexity or invasiveness of an intervention mechanism may deter an individual from using them in practice. Previous research tackled this challenge using collected motion data and conventional Machine Learning (ML) algorithms to classify heavy drinking episodes, but with impractical accuracy and computational efficiency for mobile devices. Consequently, we have elected to use Hyperdimensional Computing (HDC) to design a just-in-time intervention approach that is practical for smartphones, smart wearables, and IoT deployment. HDC is a framework that has proven results in processing real-time sensor data efficiently. This approach offers several advantages, including low latency, minimal power consumption, and high parallelism. We explore various HDC encoding designs and combine them with various HDC learning models to create an optimal and feasible approach for mobile devices. Our findings indicate an accuracy rate of 89\%, which represents a substantial 12\% improvement over the current state-of-the-art.

==> content/discussion.tex <==
\section{Discussion}
While the current findings are quite promising, there remain opportunities for improvement. A significant challenge associated with analyzing data sourced from smartphones lies in the diverse range of situations in which they are used, from being held in hand to being stored in pockets or purses. Additionally, it's conceivable that a user might not have their smartphone with them while consuming alcohol. For these reasons, this study using smart wearables like smartwatches could yield substantial gains in accuracy and improve response time in alerting users when they exceed the desired blood alcohol content.

